An Error-Guided Correction Model for Chinese Spelling Error Correction

Although existing neural network approaches have achieved great success on Chinese spelling correction, there is still room to improve. The model is required to avoid over-correction and to distinguish a correct token from its phonological and visually similar ones. In this paper, we propose an error-guided correction model (EGCM) to improve Chinese spelling correction. By borrowing the powerful ability of BERT, we propose a novel zero-shot error detection method to do a preliminary detection, which guides our model to attend more on the probably wrong tokens in encoding and to avoid modifying the correct tokens in generating. Furthermore, we introduce a new loss function to integrate the error confusion set, which enables our model to distinguish easily misused tokens. Moreover, our model supports highly parallel decoding to meet real application requirements. Experiments are conducted on widely used benchmarks. Our model achieves superior performance against state-of-the-art approaches by a remarkable margin, on both the correction quality and computation speed.

==> ori_table.tex <==
% === original table ===
\cline{2-9}
                                      & Acc.          & Pre.          & Rec.                & F1.           & Acc.          & Pre.          & Rec.                 & F1            &                      &                      &                      &                      &                      &                      &                      &                      &                      &                      &                      &                      &                       \\
\cline{1-9}
Confusionset \citeyearpar{conf/acl/WangTZ19}         & -             & 66.8          & 73.1                & 69.8          & -             & 71.5          & 59.5                 & 64.9          &                      &                      &                      &                      &                      &                      &                      &                      &                      &                      &                      &                      &                       \\
FASPell \citeyearpar{2019FASPell}                   & 74.2          & 67.6          & 60.6                & 63.5          & 73.7          & 66.6          & 59.1                 & 62.6          &                      &                      &                      &                      &                      &                      &                      &                      &                      &                      &                      &                      &                       \\
SpellGCN \citeyearpar{journals/corr/abs-2004-14166}                & -             & 74.8          & 80.7                & 77.7          & -             & 72.1          & 77.7                 & 75.9          &                      &                      &                      &                      &                      &                      &                      &                      &                      &                      &                      &                      &                       \\
Chunk2020 \citeyearpar{2020Chunk}                      & 76.8          & 88.1          & 62.0                & 72.8          & 74.6          & 87.3          & 57.6                 & 69.4          &                      &                      &                      &                      &                      &                      &                      &                      &                      &                      &                      &                      &                       \\
SM BERT \citeyearpar{conf/acl/ZhangHLL20}                  & 80.9          & 73.7          & 73.2                & 73.5          & 77.4          & 66.7          & 66.2                 & 66.4          &                      &                      &                      &                      &                      &                      &                      &                      &                      &                      &                      &                      &                       \\
RoBERTa-DCN \citeyearpar{wang2021dynamic}            & -             & 76.6          & 79.8                & 78.2          & -             & 74.2          & 77.3                 & 75.7          &                      &                      &                      &                      &                      &                      &                      &                      &                      &                      &                      &                      &                       \\
ECSpell \citeyearpar{2022General}                    & 83.4          & 76.4          & 79.9                & 78.1          & 82.4          & 74.4          & 77.9                 & 76.1          &                      &                      &                      &                      &                      &                      &                      &                      &                      &                      &                      &                      &                       \\
\cline{1-9}
PLOME^{\#} \citeyearpar{liu-etal-2021-plome}       & -             & 77.4          & 81.5                & 79.4          & -             & 75.3          & 79.3                 & 77.2          &                      &                      &                      &                      &                      &                      &                      &                      &                      &                      &                      &                      &                       \\
REALISE^{\#} \citeyearpar{2021Read}                 & 84.7          & 77.3          & 81.3                & 79.3          & 84.0          & 75.9          & 79.9                 & 77.8          &                      &                      &                      &                      &                      &                      &                      &                      &                      &                      &                      &                      &                       \\
PHMOSpell^{\#} \citeyearpar{2021PHMOSpell}          & -             & \textbf{90.1} & 72.7                & 80.5          & -             & \textbf{89.6} & 69.2                 & 78.1          &                      &                      &                      &                      &                      &                      &                      &                      &                      &                      &                      &                      &                       \\
MLM-phonetics^{\#} \citeyearpar{zhang2021correcting} & -             & 77.5          & \textbf{83.1}                & 80.2          & -             & 74.9          & \textbf{80.2}                 & 77.5          &                      &                      &                      &                      &                      &                      &                      &                      &                      &                      &                      &                      &                       \\
GAD^{\#} \citeyearpar{guo2021global}            & -             & 75.6          & 80.4                & 77.9          & -             & 73.2          & 77.8                 & 75.4          &                      &                      &                      &                      &                      &                      &                      &                      &                      &                      &                      &                      &                       \\
SpellBert^{\#} \citeyearpar{ji2021spellbert}        & -             & 87.5          & 73.6                & 80.0          & -             & 87.1          & 71.5                 & 78.5          &                      &                      &                      &                      &                      &                      &                      &                      &                      &                      &                      &                      &                       \\
\cline{1-9}
BERT-finetune                                   & 82.4          & 74.2          & 78.0                & 76.1          & 81.0          & 71.6          & 75.3                 & 73.4          & \multicolumn{1}{c}{} & \multicolumn{1}{c}{} & \multicolumn{1}{c}{} & \multicolumn{1}{c}{} & \multicolumn{1}{c}{} & \multicolumn{1}{c}{} & \multicolumn{1}{c}{} & \multicolumn{1}{c}{} & \multicolumn{1}{c}{} & \multicolumn{1}{c}{} & \multicolumn{1}{c}{} & \multicolumn{1}{c}{} & \multicolumn{1}{c}{}  \\
Our EGCM                                   & 86.4          & 82.7          & 77.6                & 80.0          & 85.8          & 80.6          & 74.7                 & 77.5          &                      &                      &                      &                      &                      &                      &                      &                      &                      &                      &                      &                      &                       \\
Pre-Tn EGCM^{\#}                             & \textbf{87.2} & 83.4          & 79.8                & \textbf{81.6} & \textbf{86.3} & 81.4          & 78.4                 & \textbf{79.9} &                      &                      &                      &                      &                      &                      &                      &                      &                      &                      &                      &                      &                       \\
